Mechanized HOL Reasoning in Set Theory

We present a mechanized embedding of higher-order logic (HOL) and algebraic data types (ADT) into first-order logic with ZFC axioms. We implement this in the Lisa proof assistant for schematic first-order logic and its library based on axiomatic set theory. HOL proof steps are implemented as proof producing tactics in Lisa, and the types are interpreted as sets, with function (or arrow) types coinciding with set-theoretic function spaces. The embedded HOL proofs, as opposed to being a layer over the existing proofs, are interoperable with the existing library. This yields a form of soft type system supporting top-level polymorphism and ADTs over set theory, and offer tools to reason about functions in set theory.

==> related.tex <==
% related.tex
% related work

% base 
% TODO: trim?
\cite{gordonSetTheoryHigher1996} provides a summary of possible approaches to combining higher-order logic and set theory, discussing both directions. It already highlights some of the challenges faced in translation during the present work, but uses Hilbert's $\epsilon$ operator to represent abstractions.
\cite{Obus2015Type,agerholm1995Experiments} study axiomatization of set theory within higher-order logic based proof assistants.
\cite{Kaliszyk2023Combining} define Tarski-Grothendieck set theory as an Isabelle logic, and import in it theorems from both Isabelle/HOL and Isabelle/Mizar. \cite{Brown2006Combining} presents a dependent type theory supporting MacLane set theory, where sets and classes can be used as types. 

% opentheory and HOL -> set theory
OpenTheory \cite{hurd2011opentheory} is an interchange format for higher-order
logic based provers, based on the core theory of the HOL family of provers,
implementing bidirectional translation between several provers.
\cite{carneiro2016conversion} presents a translation of OpenTheory articles into
the Metamath system and uses it to import theorems from HOL Light into it, with ZFC axiomatization.

In the present work we picked HOL Light as our reference system for HOL, but with some additional work, the results can be translated to other proof assistants in the HOL-family of proof assistants, such as HOL4 \cite{slindBriefOverviewHOL42008}, Isabelle/HOL \cite{nipkowIsabelleHOLProof2002}, or Candle \cite{abrahamssonCandleVerifiedImplementation2022}.

Similarly, our target system was Lisa, but none of the results are specific to Lisa, and they transfer to any system using axiomatic set theory over first-order logic, though those are not quite as common, such as Mizar\cite{naumowiczBriefOverviewMizar2009}.

